Du chaos dans la musique des etoiles

La plupart des etoiles variables qui pulsent avec grande amplitude, telles les cepheides, ont un comportement tres regulier et periodique. Mais juste a cote d'elles dans le diagramme Hertzsprung-Russell, se trouve un groupe d'etoiles variables dotees de courbes de lumiere tres irregulieres. A l'aide d'une technique de reconstruction de flot appliquee aux donnees d'observation astronomiques de plusieurs de ces etoiles, on montre que la dynamique sous-jacente est chaotique et de faible dimension, ce qui peut surprendre a cause de la violence de ces pulsations. En plus a l'aide d'une linearisation du flot on deduit que le mecanisme physique de la pulsation consiste en l'interaction entre deux modes vibratoires (vraisemblablement radiaux), l'un lineairement instable, de frequence f_0, et l'autre stable, mais de frequence \~2f_0 (soit un scenario a la Shilnikoff generalise).

==> abstract_english.tex <==
Translation:

Most variable stars that pulsate with large amplitudes, such as the Cepheids,
exhibit a regular, periodic behavior.  But just next to them in the 
Hertzsprung-Russell diagram exists a group of variable stars with quite
irregular light curves.  Applying a global flow reconstruction technique
to the observational light curves of some of these stars we demonstrate 
that the underlying dynamics is chaotic and of low dimension, which may
be astonishing given the violence of the pulsations. Furthermore, 
linearizing the flow around the equilibrium we show that the physical 
mechanism of the pulsation consists of the nonlinear interaction of two
(likely radial) pulsation modes, the first linearly unstable, with 
frequency f_0, and the second, linearly stable with ~2f_0 (reminiscent 
of a generalized Shilnikov scenario). 

